Cloud and Star Formation in Spiral Arms

We present the results from simulations of GMC formation in spiral galaxies. First we discuss cloud formation by cloud-cloud collisions, and gravitational instabilities, arguing that the former is prevalent at lower galactic surface densities and the latter at higher. Cloud masses are also limited by stellar feedback, which can be effective before clouds reach their maximum mass. We show other properties of clouds in simulations with different levels of feedback. With a moderate level of feedback, properties such as cloud rotations and virial parameters agree with observations. Without feedback, an unrealistic population of overly bound clouds develops. Spiral arms are not found to trigger star formation, they merely gather gas into more massive GMCs. We discuss in more detail interactions of clouds in the ISM, and argue that these are more complex than early ideas of cloud-cloud collisions. Finally we show ongoing work to determine whether the Milky Way is a flocculent or grand design spiral.

==> captions.tex <==
\caption{Example simulation of a galaxy with an $m=2$ imposed spiral potential. The simulation includes self gravity, cooling and heating of the ISM and stellar feedback (producing a multiphase ISM), but not magnetic fields. Dense regions shown by yellow in the colour table correspond to molecular clouds.}
\caption{Properties of clouds are shown from simulations in Dobbs et al. 2011. The top left panel shows the fraction of retrograde clouds versus the level of stellar feedback. The top right panel shows mass spectra for different levels of feedback. The lower panels show the virial parameter when $\epsilon=0.01$ (left, minimal feedback) and 0.05 (right, moderate feedback).}
\caption{The evolution of a $2\times10^6$ M$_{\odot}$ GMC (coloured red) is shown over a 40 Myr time period. Other clouds which coalesce with this GMC, or are the result of dispersal of the GMC, are shown in other bold colours. The locus of the gas which is situated in the chosen GMC at 250 Myr (middle panel) is indicated by the white dashed lines in the other panels. The total amount of gas in `clouds' is indicated on the top left of each panel, whilst the rest of the gas is more diffuse.}
\caption{The star formation rate is shown for simulations with different feedback efficiencies (left) and with and without a spiral potential (right). The red lines are for $\epsilon=0.05$ and the blue $\epsilon=0.1$. The black dots on the left panel are observations from Kennicutt 2008.}
\caption{Results are shown for a hydrodynamical model of a possible Milky Way, with a bar and 2 spiral arms with pitch angle $12.5^\circ$, and spiral arm pattern speed of 15 km/s/kpc. The map of CO emission for the model is shown on the right. The structure compared to actual observations (Dame et al. 2001) is in reasonable agreement, but the Carina arm is at the wrong velocities. We were unable to find a model which reproduced the full structure of the Milky Way with fixed potentials. From Pettitt et al. 2014.}

